Carnegie Supernova Project: The First Homogeneous Sample of "Super-Chandrasekhar Mass"/2003fg-like Type Ia Supernova

We present a multi-wavelength photometric and spectroscopic analysis of thirteen "Super-Chandrasekhar Mass"/2003fg-like type Ia Supernova (SNe~Ia). Nine of these objects were observed by the Carnegie Supernova Project. 2003fg-like have slowly declining light curves ($\Delta m_{15}$(B) $<$1.3 mag), and peak absolute $B$-band magnitudes between $-19<M_{B}<-21$~mag. Many 2003fg-like are located in the same part of the luminosity width relation as normal SNe~Ia. In the optical $B$ and $V$ bands, 2003fg-like look like normal SNe~Ia, but at redder wavelengths they diverge. Unlike other luminous SNe~Ia, 2003fg-like generally have only one $i$-band maximum which peaks after the epoch of $B$-band maximum, while their NIR light curve rise times can be $\gtrsim$40 days longer than those of normal SNe~Ia. They are also at least one magnitude brighter in the NIR bands than normal SNe~Ia, peaking above $M_H < -19$~mag, and generally have negative Hubble residuals, which may be the cause of some systematics in dark energy experiments. Spectroscopically, 2003fg-like exhibit peculiarities such as unburnt carbon well past maximum light, a large spread (8000--12000~km/s) in SiII $\lambda$6355 velocities at maximum light with no rapid early velocity decline, and no clear $H$-band break at +10~d, e. We find that SNe with a larger pseudo equivalent width of CII at maximum light have lower SiII $\lambda$6355 velocities and slower declining light curves. There are also multiple factors that contribute to the peak luminosity of 2003fg-like. The explosion of a C-O degenerate core inside a carbon-rich envelope is consistent with these observations. Such a configuration may come from the core degenerate scenario.

==> ref.tex <==
\begin{thebibliography}{}
\bibitem[Ashall et al.(2020)]{Ashall20} Ashall, C., Lu, J., Burns, C., et al.\ 2020, \apjl, 895, L3

\bibitem[Ashall et al.(2019a)]{Ashall19a} Ashall, C., Hsiao, E.~Y., Hoeflich, P., et al.\ 2019a, \apjl, 875, L14

\bibitem[Ashall et al.(2019b)]{Ashall19b} Ashall, C., Hoeflich, P., Hsiao, E.~Y., et al.\ 2019b, \apj, 878, 86

\bibitem[\protect\citeauthoryear{Ashall, et al.}{2018}]{Ashall18} Ashall C., et al., 2018, MNRAS, 477, 153

\bibitem[Ashall et al.(2016)]{Ashall16b} Ashall, C., Mazzali, P.~A., Pian, E., et al.\ 2016, \mnras, 463, 1891

\bibitem[Baltay et al.(2013)]{Baltay13} Baltay, C., Rabinowitz, D., Hadjiyska, E., et al.\ 2013, \pasp, 125, 683. doi:10.1086/671198

\bibitem[Benitez et al.(2014)]{Benitez14} Benitez, S., Polshaw, J., Inserra, C., et al.\ 2014, The Astronomer's Telegram, 6118

\bibitem[\protect\citeauthoryear{Branch, et al.}{2006}]{Branch06} Branch D., et al., 2006, PASP, 118, 560

\bibitem[Brown et al.(2014)]{Brown14} Brown, P.~J., Kuin, P., Scalzo, R., et al.\ 2014, \apj, 787, 29

\bibitem[Blondin et al.(2012)]{Blondin12} Blondin, S., Matheson, T., Kirshner, R.~P., et al.\ 2012, \aj, 143, 126. doi:10.1088/0004-6256/143/5/126

\bibitem[Burns et al.(2018)]{Burns18} Burns, C.~R., Parent, E., Phillips, M.~M., et al.\ 2018, \apj, 869, 56. doi:10.3847/1538-4357/aae51c


\bibitem[\protect\citeauthoryear{Burns, et al.}{2014}]{Burns14} Burns C.~R., et al., 2014, ApJ, 789, 32

\bibitem[Burns et al.(2011)]{Burns11} Burns, C.~R., Stritzinger, M., Phillips, M.~M., et al.\ 2011, \aj, 141, 19

\bibitem[Burrow et al.(2020)]{Burrow20} Burrow, A., Baron, E., Ashall, C., et al.\ 2020, arXiv:2008.07636


\bibitem[Cappellaro et al.(2001)]{Cappellaro01} Cappellaro, E., Patat, F., Mazzali, P.~A., et al.\ 2001, \apjl, 549, L215

\bibitem[Childress et al.(2011)]{Childress11} Childress, M., Aldering, G., Aragon, C., et al.\ 2011, \apj, 733, 3. doi:10.1088/0004-637X/733/1/3


\bibitem[Cikota et al.(2019)]{Cikota19} Cikota, A., Patat, F., Wang, L., et al.\ 2019, \mnras, 490, 578

\bibitem[Chakradhari et al.(2014)]{Chakradhari14} Chakradhari, N.~K., Sahu, D.~K., Srivastav, S., et al.\ 2014, \mnras, 443, 1663

\bibitem[\protect\citeauthoryear{Chen, et al.}{2019}]{Chen19} Chen P., et al., 2019, ApJ, 880, 35

\bibitem[Das \& Mukhopadhyay(2013)]{Das13} Das, U. \& Mukhopadhyay, B.\ 2013, \prl, 110, 071102. doi:10.1103/PhysRevLett.110.071102

\bibitem[Dessart et al.(2014)]{Dessart14} Dessart, L., Hillier, D.~J., Blondin, S., et al.\ 2014, \mnras, 439, 3114

\bibitem[Drake et al.(2009)]{Drake09} Drake, A.~J., Djorgovski, S.~G., Mahabal, A., et al.\ 2009, \apj, 696, 870. doi:10.1088/0004-637X/696/1/870

\bibitem[Drake et al.(2013)]{Drake13} Drake, A.~J., Djorgovski, S.~G., Graham, M.~J., et al.\ 2013, Central Bureau Electronic Telegrams, 3442

\bibitem[Filippenko et al.(1992a)]{Filippenko91bg} Filippenko, A.~V., Richmond, M.~W., Branch, D., et al.\ 1992a, \aj, 104, 1543

\bibitem[Filippenko et al.(1992b)]{Filippenko92} Filippenko, A.~V., Richmond, M.~W., Matheson, T., et al.\ 1992b, \apjl, 384, L15

\bibitem[Firth et al.(2015)]{Firth15} Firth, R.~E., Sullivan, M., Gal-Yam, A., et al.\ 2015, \mnras, 446, 3895. doi:10.1093/mnras/stu2314

\bibitem[Fleury et al.(2014)]{Fleury14} Fleury, M., Leget, P.-F., Le Guillou, L., et al.\ 2014, The Astronomer's Telegram, 5720

\bibitem[Folatelli et al.(2013)]{Folatelli13} Folatelli, G., Morrell, N., Phillips, M.~M., et al.\ 2013, \apj, 773, 53

\bibitem[\protect\citeauthoryear{Foley, et al.}{2013}]{Foley13} Foley R.~J., et al., 2013, ApJ, 767, 57

\bibitem[Foley et al.(2010)]{Foley10} Foley, R.~J., Narayan, G., Challis, P.~J., et al.\ 2010, \apj, 708, 1748

\bibitem[Friesen et al.(2017)]{Friesen17} Friesen, B., Baron, E., Parrent, J.~T., et al.\ 2017, \mnras, 467, 2392. doi:10.1093/mnras/stx241


\bibitem[Galbany et al.(2021)]{Galbany21} Galbany, L., Ashall, C., + in prep

\bibitem[Galbany et al.(2019)]{Galbany19} Galbany, L., Ashall, C., H{\"o}flich, P., et al.\ 2019, \aap, 630, A76

\bibitem[Gall et al.(2018)]{Gall18} Gall, C., Stritzinger, M.~D., Ashall, C., et al.\ 2018, \aap, 611, A58

\bibitem[Ganeshalingam et al.(2012)]{Ganeshalingam12} Ganeshalingam, M., Li, W., Filippenko, A.~V., et al.\ 2012, \apj, 751, 142. doi:10.1088/0004-637X/751/2/142

\bibitem[Garavini et al.(2007)]{Garavini07} Garavini, G., Folatelli, G., Nobili, S., et al.\ 2007, \aap, 470, 411

\bibitem[Gonz{\'a}lez-Gait{\'a}n et al.(2014)]{Gonzalez14} Gonz{\'a}lez-Gait{\'a}n, S., Hsiao, E.~Y., Pignata, G., et al.\ 2014, \apj, 795, 142. doi:10.1088/0004-637X/795/2/142

\bibitem[Graham et al.(2017)]{Graham17} Graham, M.~L., Kumar, S., Hosseinzadeh, G., et al.\ 2017, \mnras, 472, 3437. doi:10.1093/mnras/stx2224

\bibitem[Hachinger et al.(2012)]{Hachinger12} Hachinger, S., Mazzali, P.~A., Taubenberger, S., et al.\ 2012, \mnras, 427, 2057

\bibitem[Hachinger et al.(2008)]{Hachinger08} Hachinger, S., Mazzali, P.~A., Tanaka, M., et al.\ 2008, \mnras, 389, 1087

\bibitem[Hammer et al.(2010)]{Hammer10} Hammer, D., Verdoes Kleijn, G., Hoyos, C., et al.\ 2010, \apjs, 191, 143. doi:10.1088/0067-0049/191/1/143

\bibitem[Hamuy et al.(2006)]{Hamuy06} Hamuy, M., Folatelli, G., Morrell, N.~I., et al.\ 2006, \pasp, 118, 2

\bibitem[Hicken et al.(2007)]{Hicken07} Hicken, M., Garnavich, P.~M., Prieto, J.~L., et al.\ 2007, \apjl, 669, L17

\bibitem[H{\"o}flich et al.(2002)]{Hoeflich02} H{\"o}flich, P., Gerardy, C.~L., Fesen, R.~A., et al.\ 2002, \apj, 568, 791

\bibitem[Hoeflich, \& Khokhlov(1996)]{hk96} Hoeflich, P., \& Khokhlov, A.\ 1996, \apj, 457, 500

\bibitem[Howell et al.(2006)]{Howell06} Howell, D.~A., Sullivan, M., Nugent, P.~E., et al.\ 2006, \nat, 443, 308

\bibitem[Hsiao et al.(2007)]{Hsiao07} Hsiao, E.~Y., Conley, A., Howell, D.~A., et al.\ 2007, \apj, 663, 1187

\bibitem[Hsiao et al.(2013)]{Hsiao13} Hsiao, E.~Y., Marion, G.~H., Phillips, M.~M., et al.\ 2013, \apj, 766, 72. doi:10.1088/0004-637X/766/2/72

\bibitem[Hsiao et al.(2015)]{Hsiao15} Hsiao, E.~Y., Burns, C.~R., Contreras, C., et al.\ 2015, \aap, 578, A9

\bibitem[Hsiao et al.(2019)]{Hsiao19} Hsiao, E.~Y., Phillips, M.~M., Marion, G.~H., et al.\ 2019, \pasp, 131, 014002. doi:10.1088/1538-3873/aae961

\bibitem[Hsiao et al.(2020)]{Hsiao20} Hsiao, E.~Y., Hoeflich, P., Ashall, C., et al.\ 2020, \apj, 900, 140. doi:10.3847/1538-4357/abaf4c

\bibitem[Iben \& Tutukov(1984)]{Iben84} Iben, I. \& Tutukov, A.~V.\ 1984, \apjs, 54, 335. doi:10.1086/190932

\bibitem[Inserra et al.(2013)]{Inserra13} Inserra, C., Nicholl, M., Walton, N., et al.\ 2013, The Astronomer's Telegram, 4863

\bibitem[Jack et al.(2015)]{Jack15} Jack, D., Baron, E., \& Hauschildt, P.~H.\ 2015, \mnras, 449, 3581

\bibitem[Jiang et al.(2018)]{Jiang18} Jiang, J.-. an ., Doi, M., Maeda, K., et al.\ 2018, \apj, 865, 149. doi:10.3847/1538-4357/aadb9a

\bibitem[Kashi \& Soker(2011)]{Kashi11} Kashi, A. \& Soker, N.\ 2011, \mnras, 417, 1466. doi:10.1111/j.1365-2966.2011.19361.x


\bibitem[Kasen(2006)]{Kasen06} Kasen, D.\ 2006, \apj, 649, 939

\bibitem[Kirshner et al.(1973)]{Kirshner73} Kirshner, R.~P., Willner, S.~P., Becklin, E.~E., et al.\ 1973, \apjl, 180, L97

\bibitem[Kochanek et al.(2017)]{Kochanek17} Kochanek, C.~S., Shappee, B.~J., Stanek, K.~Z., et al.\ 2017, \pasp, 129, 104502. doi:10.1088/1538-3873/aa80d9

\bibitem[Kromer et al.(2015)]{Kromer15} Kromer, M., Ohlmann, S.~T., Pakmor, R., et al.\ 2015, \mnras, 450, 3045. doi:10.1093/mnras/stv886

\bibitem[Krisciunas et al.(2017)]{Krisciunas17} Krisciunas, K., Contreras, C., Burns, C.~R., et al.\ 2017, \aj, 154, 211

\bibitem[Lentz et al.(2000)]{Lentz00} Lentz, E.~J., Baron, E., Branch, D., et al.\ 2000, \apj, 530, 966

\bibitem[Li et al.(2003)]{Li03} Li, W., Filippenko, A.~V., Chornock, R., et al.\ 2003, \pasp, 115, 453

\bibitem[Leibundgut et al.(1993)]{Leibundgut93} Leibundgut, B., Kirshner, R.~P., Phillips, M.~M., et al.\ 1993, \aj, 105, 301

\bibitem[Lira et al.(1998)]{Lira98} Lira, P., Suntzeff, N.~B., Phillips, M.~M., et al.\ 1998, \aj, 115, 234

\bibitem[Livne(1990)]{Livne90} Livne, E.\ 1990, \apjl, 354, L53. doi:10.1086/185721

\bibitem[Lu et al.(2021)]{Lu21} Lu, J., Ashall, C., Hsiao, E, et al.\ 2021, \aj, XXX.XXX

\bibitem[Maeda et al.(2009)]{Maeda09} Maeda, K., Kawabata, K., Li, W., et al.\ 2009, \apj, 690, 1745

\bibitem[Maguire et al.(2012)]{Maguire12} Maguire, K., Pan, Y., Le Guillou, L., et al.\ 2012, The Astronomer's Telegram, 4624

\bibitem[Marion et al.(2009)]{Marion09} Marion, G.~H., H{\"o}flich, P., Gerardy, C.~L., et al.\ 2009, \aj, 138, 727

\bibitem[Masci et al.(2017)]{Masci17} Masci, F.~J., Laher, R.~R., Rebbapragada, U.~D., et al.\ 2017, \pasp, 129, 014002. doi:10.1088/1538-3873/129/971/014002

\bibitem[Mazzali et al.(2014)]{Mazzali14} Mazzali, P.~A., Sullivan, M., Hachinger, S., et al.\ 2014, \mnras, 439, 1959

\bibitem[Mazzali \& Hachinger(2012)]{Mazzali12} Mazzali, P.~A. \& Hachinger, S.\ 2012, \mnras, 424, 2926

\bibitem[Mazzali et al.(2008)]{Mazzali08} Mazzali, P.~A., Sauer, D.~N., Pastorello, A., et al.\ 2008, \mnras, 386, 1897

\bibitem[Mazzali(2000)]{Mazzali00} Mazzali, P.~A.\ 2000, \aap, 363, 705

\bibitem[Miller et al.(2020)]{Miller20} Miller, A.~A., Magee, M.~R., Polin, A., et al.\ 2020, arXiv e-prints, arXiv:2005.05972

\bibitem[Morokuma et al.(2014)]{Morokuma14} Morokuma, T., Tominaga, N., Tanaka, M., et al.\ 2014, \pasj, 66, 114. doi:10.1093/pasj/psu105

\bibitem[Mould et al.(2000)]{Mould00} Mould, J.~R., Huchra, J.~P., Freedman, W.~L., et al.\ 2000, \apj, 529, 786. doi:10.1086/308304

\bibitem[Noebauer et al.(2016)]{Noebauer16} Noebauer, U.~M., Taubenberger, S., Blinnikov, S., et al.\ 2016, \mnras, 463, 2972. doi:10.1093/mnras/stw2197

\bibitem[Nagao et al.(2018)]{Nagao18} Nagao, T., Maeda, K., \& Yamanaka, M.\ 2018, \mnras, 476, 4806. doi:10.1093/mnras/sty538

\bibitem[Nagao et al.(2017)]{Nagao17} Nagao, T., Maeda, K., \& Yamanaka, M.\ 2017, \apj, 835, 143. doi:10.3847/1538-4357/835/2/143

\bibitem[Nakano et al.(2015)]{Nakano15} Nakano, S., Itagaki, K., \& Lucey, J.~R.\ 2015, Central Bureau Electronic Telegrams, 4123

\bibitem[Parrent et al.(2016)]{Parrent16} Parrent, J.~T., Howell, D.~A., Fesen, R.~A., et al.\ 2016, \mnras, 457, 3702

\bibitem[Perlmutter et al.(1999)]{Perlmutter99} Perlmutter, S., Aldering, G., Goldhaber, G., et al.\ 1999, \apj, 517, 565. doi:10.1086/307221


\bibitem[\protect\citeauthoryear{Phillips, et al.}{2019}]{Phillips19} Phillips M.~M., et al., 2019, PASP, 131, 014001

\bibitem[Phillips et al.(2013)]{Phillips13} Phillips, M.~M., Simon, J.~D., Morrell, N., et al.\ 2013, \apj, 779, 38

\bibitem[Phillips et al.(1999)]{Phillips99} Phillips, M.~M., Lira, P., Suntzeff, N.~B., et al.\ 1999, \aj, 118, 1766

\bibitem[Phillips(1993)]{Phillips93} Phillips, M.~M.\ 1993, \apjl, 413, L105. doi:10.1086/186970

\bibitem[Phillips et al.(1992)]{Phillips92} Phillips, M.~M., Wells, L.~A., Suntzeff, N.~B., et al.\ 1992, \aj, 103, 1632


\bibitem[Phillips et al.(1987)]{Phillips87} Phillips, M.~M., Phillips, A.~C., Heathcote, S.~R., et al.\ 1987, \pasp, 99, 592


\bibitem[Poznanski et al.(2012)]{Poznanski12} Poznanski, D., Prochaska, J.~X., \& Bloom, J.~S.\ 2012, \mnras, 426, 1465

\bibitem[Pskovskii(1984)]{Pskovskii84} Pskovskii, Y.~P.\ 1984, \sovast, 28, 658

\bibitem[Quimby et al.(2006)]{Quimby06} Quimby, R., H{\"o}flich, P., Kannappan, S.~J., et al.\ 2006, \apj, 636, 400. doi:10.1086/498014

\bibitem[Riess et al.(1998)]{Riess98} Riess, A.~G., Filippenko, A.~V., Challis, P., et al.\ 1998, \aj, 116, 1009. doi:10.1086/300499

\bibitem[Sand et al.(2019)]{Sand19} Sand, D.~J., Amaro, R.~C., Moe, M., et al.\ 2019, \apjl, 877, L4

\bibitem[Scalzo et al.(2014)]{Scalzo14} Scalzo, R.~A., Childress, M., Tucker, B., et al.\ 2014, \mnras, 445, 30

\bibitem[Scalzo et al.(2010)]{Scalzo10} Scalzo, R.~A., Aldering, G., Antilogus, P., et al.\ 2010, \apj, 713, 1073

\bibitem[\protect\citeauthoryear{Schlafly \& Finkbeiner}{2011}]{Schlafly11} Schlafly E.~F., Finkbeiner D.~P., 2011, ApJ, 737, 103

\bibitem[Shappee et al.(2014)]{Shappee14} Shappee, B.~J., Prieto, J.~L., Grupe, D., et al.\ 2014, \apj, 788, 48. doi:10.1088/0004-637X/788/1/48

\bibitem[Silverman et al.(2011)]{Silverman11} Silverman, J.~M., Ganeshalingam, M., Li, W., et al.\ 2011, \mnras, 410, 585

\bibitem[Simcoe et al.(2013)]{Simcoe13} Simcoe, R.~A., Burgasser, A.~J., Schechter, P.~L., et al.\ 2013, \pasp, 125, 270. doi:10.1086/670241

\bibitem[Smartt et al.(2015)]{Smartt15} Smartt, S.~J., Valenti, S., Fraser, M., et al.\ 2015, \aap, 579, A40. doi:10.1051/0004-6361/201425237

\bibitem[Taubenberger et al.(2019)]{Taubenberger19} Taubenberger, S., Floers, A., Vogl, C., et al.\ 2019, \mnras, 488, 5473

\bibitem[Taubenberger et al.(2013a)]{Taubenberger13a} Taubenberger, S., Kromer, M., Hachinger, S., et al.\ 2013, \mnras, 432, 3117

\bibitem[Taubenberger et al.(2013b)]{Taubenberger:2013b} Taubenberger, S., Kromer, M., Pakmor, R., et al.\ 2013, \apjl, 775, L43

\bibitem[Taubenberger et al.(2011)]{Taubenberger11} Taubenberger, S., Benetti, S., Childress, M., et al.\ 2011, \mnras, 412, 2735

\bibitem[Tanaka et al.(2010)]{Tanaka10} Tanaka, M., Kawabata, K.~S., Yamanaka, M., et al.\ 2010, \apj, 714, 1209

\bibitem[Turatto et al.(2003)]{Turatto03} Turatto, M., Benetti, S., \& Cappellaro, E.\ 2003, From Twilight to Highlight: The Physics of Supernovae, 200. doi:10.1007/10828549$\_$26


\bibitem[Yamanaka et al.(2016)]{Yamanaka16} Yamanaka, M., Maeda, K., Tanaka, M., et al.\ 2016, \pasj, 68, 68. doi:10.1093/pasj/psw047

\bibitem[Yamanaka et al.(2009)]{Yamanaka09} Yamanaka, M., Kawabata, K.~S., Kinugasa, K., et al.\ 2009, \apjl, 707, L118

\bibitem[Yoon \& Langer(2005)]{Yoon05} Yoon, S.-C. \& Langer, N.\ 2005, \aap, 435, 967. doi:10.1051/0004-6361:20042542


\bibitem[Yuan et al.(2010)]{Yuan10} Yuan, F., Quimby, R.~M., Wheeler, J.~C., et al.\ 2010, \apj, 715, 1338

\bibitem[Walker et al.(2015)]{Walker15} Walker, E.~S., Baltay, C., Campillay, A., et al.\ 2015, \apjs, 219, 13. doi:10.1088/0067-0049/219/1/13

\bibitem[Whelan \& Iben(1973)]{Whelan73} Whelan, J. \& Iben, I.\ 1973, \apj, 186, 1007. doi:10.1086/152565


\bibitem[Wheeler et al.(1998)]{Wheeler98} Wheeler, J.~C., H{\"o}flich, P., Harkness, R.~P., et al.\ 1998, \apj, 496, 908

\bibitem[Zhang et al.(2016)]{Zhang16} Zhang, J.-J., Wang, X.-F., Sasdelli, M., et al.\ 2016, \apj, 817, 114

\end{thebibliography}

